SpecFit: Not All Draft Tokens Cost the Same in Offloaded MoE Inference

Mixture-of-experts (MoE) models activate only a few experts per token, but when their expert weights are offloaded to host memory, host-to-device (H2D) expert transfers enter the critical path of decoding. Speculative decoding verifies several draft tokens in one forward pass, yet in an MoE model each verified token activates its own experts, so a larger draft tree transfers more experts. Because of this H2D cost, speculative decoding commits several tokens per verification cycle yet is sometimes even slower than autoregressive decoding. Based on this observation, we propose SpecFit, which chooses the verified draft subtree to maximize predicted throughput rather than acceptance length. SpecFit estimates the expected number of committed tokens from draft path probabilities and predicts cycle time from the node count and the per-layer union of the experts the subtree activates; this union is a monotone submodular coverage function, so each node pays only for the experts it adds. An exact search over ancestor-closed subtrees returns the subtree with the highest predicted throughput; run after each draft level, the same search also decides when to stop drafting, and the unmodified target verifies the result. On CNN/DailyMail summarization and a GSM8K subset with Qwen3-30B-A3B, SpecFit decodes 21.6% and 7.0% faster than EAGLE-3 with the same expert cache and 1.97x and 1.72x as fast as vanilla EAGLE-3. Code is available at https://github.com/Chlience/SpecFit.

==> fig-bars.tex <==
% Shared bar-chart style for Figures fig:summ, fig:gsm8k, fig:slots, and fig:slots-mechanism (main.tex and main-zh.tex).
% Decode TPS (unless a figure sets its own label) on the y axis from zero with light grid lines; the value sits on each bar.
% SpecFit blue, EAGLE-3 gray, AR light gray with a frame; the legend runs above the axis.
\definecolor{ovblue}{HTML}{0072B2}
\pgfplotsset{
  tpsbar/.style={
    ybar=3pt, bar width=22pt, scale only axis, height=2.5cm, ymin=0,
    ymajorgrids, grid style={black!12, line width=0.3pt},
    axis x line*=bottom, axis y line*=left, axis line style={black!60},
    tick style={black!60}, major x tick style={draw=none},
    tick label style={font=\sffamily\scriptsize, /pgf/number format/assume math mode=true},
    label style={font=\sffamily\scriptsize},
    ylabel={\enzh{Decode TPS}{解码 TPS}}, ylabel style={yshift=-2pt},
    nodes near coords,
    every node near coord/.append style={font=\sffamily\scriptsize, inner sep=1.5pt,
      anchor=south, fill=white, /pgf/number format/fixed, /pgf/number format/fixed zerofill,
      /pgf/number format/precision=2, /pgf/number format/assume math mode=true},
    legend style={font=\sffamily\scriptsize, draw=none, fill=none, legend columns=-1,
      at={(0.5,1.03)}, anchor=south, /tikz/every even column/.append style={column sep=8pt}},
    legend image code/.code={\draw[#1] (0cm,-0.08cm) rectangle (0.24cm,0.1cm);},
  },
  specfit/.style={fill=ovblue, draw=none},
  eagle/.style={fill=black!28, draw=none},
  arbar/.style={fill=black!7, draw=black!50, line width=0.4pt},
}

